SYNAPSE-G: Bridging Large Language Models and Graph Learning for Rare Event Classification

Scarcity of labeled data, especially for rare events, hinders training effective machine learning models. This paper proposes SYNAPSE-G (Synthetic Augmentation for Positive Sampling via Expansion on Graphs), a novel pipeline leveraging Large Language Models (LLMs) to generate synthetic training data for rare event classification, addressing the cold-start problem. This synthetic data serve as seeds for semi-supervised label propagation on a similarity graph constructed between the seeds and a large unlabeled dataset. This identifies candidate positive examples, subsequently labeled by an oracle (human or LLM). The expanded dataset then trains/fine-tunes a classifier. We theoretically analyze how the quality (validity and diversity) of the synthetic data impacts the precision and recall of our method. Experiments on the imbalanced SST2 and MHS datasets demonstrate SYNAPSE-G's effectiveness in finding positive labels, outperforming baselines including nearest neighbor search.

==> sections/enlarged.tex <==
\begin{figure*}[t!]
\centering
\begin{subfigure}[t]{0.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/fig-1.pdf}
  \caption{\small Precision v. Recall}
  \label{fig:image1-en}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/fig-2.pdf}
  \caption{\small Recall v. Query Ratio}
  \label{fig:image2-en}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/fig-3.pdf}
  \caption{\small Precision v. Query Ratio}
  \label{fig:image3-en}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/fig-4.pdf}
      \caption{\small F1 Score v. Query Ratio}
    \label{fig:image4-en}
\end{subfigure}

\caption{\small [Enlarged version of Figure~\ref{fig:combined_results}] Experimental results on the imbalanced SST2 dataset. (a) Precision v. Recall comparing ACS and random seed selection. (b) Recall v. Query Ratio, (c) Precision v. Query Ratio and (d) F1 Score v. Query Ratio, showing the impact of parameters. %ACS consistently outperforms random seed selection across all metrics. Figures (b), (c), and (d) demonstrate the impact of varying similarity thresholds and maximum degree constraints.
 Curves above the expected random performance indicate a benefit of the graph-based approach.}
\label{fig:combined_results-enlarged}
\end{figure*}
